Understanding the efficacy, reliability and resiliency of computer vision techniques for malware detection and future research directions

My research lies in the intersection of security and machine learning. This overview summarizes one component of my research: combining computer vision with malware exploit detection for enhanced security solutions. I will present the perspectives of efficacy, reliability and resiliency to formulate threat detection as computer vision problems and develop state-of-the-art image-based malware classification. Representing malware binary as images provides a direct visualization of data samples, reduces the efforts for feature extraction, and consumes the whole binary for holistic structural analysis. Employing transfer learning of deep neural networks effective for large scale image classification to malware classification demonstrates superior classification efficacy compared with classical machine learning algorithms. To enhance reliability of these vision-based malware detectors, interpretation frameworks can be constructed on the malware visual representations and useful for extracting faithful explanation, so that security practitioners have confidence in the model before deployment. In cyber-security applications, we should always assume that a malware writer constantly modifies code to bypass detection. Addressing the resiliency of the malware detectors is equivalently important as efficacy and reliability. Via understanding the attack surfaces of machine learning models used for malware detection, we can greatly improve the robustness of the algorithms to combat malware adversaries in the wild. Finally I will discuss future research directions worth pursuing in this research community.

==> dynamic.tex <==
\section{Transfer Learning on Image Series for Dynamic Analysis}
we investigate more sophisticated dynamic features to build robust deep learning malware classifier. In this paper, we describe a malware detection system based on hierarchical ensemble neural network, HeNet, that classifies the control flow trace of an execution. Control flow analysis has been widely used in security to mitigate memory corruption attacks by enforcing pre-specified security policies over a program execution~\cite{Abadi09}. HeNet, however, is the first malware detection approach to apply deep learning on fine-grained control flow traces.  We build a per-application deep-learning behavioral model to distinguish benign and malicious executions of the application. The key observation underlying our work is that malware exploits temporarily or persistently execute malicious code in the context of a victim application and hence, change the original control flow of the application. %to execute non-native code. 

We utilize Intel\textsuperscript{\textregistered} Processor Trace (Intel\textsuperscript{\textregistered} PT), a low overhead tracing hardware, to get the complete control flow of a program execution. Intel\textsuperscript{\textregistered} PT records the non-deterministic control flow transfers, contextual, timing, etc. information and transmits the data in highly compressed trace packets. The control flow packets combined with the program binary can be used to reconstruct the exact sequence of instructions executed but the post-processing takes a long time due to the high volume of trace data. We, however, notice that the control flow packets can be used as an encoded representation of the control flow transfers over a program execution. We convert the payload of control flow packets to a stream of pixels and represent the control flow as a time series of images. Utilizing low level trace packets eliminates manual feature engineering and makes our system portable across different operating systems and hardware.

\begin{table} 
\centering
  \label{tab:comparison}
  \caption{Comparison of HeNet with other classifiers}
  \begin{tabular}{||l|l|l|l||}
  \hline
    Behavior model &  Accuracy & FPR & Resolution \\ \hline  
     HeNet low-level model & 0.98 & 0.0073 & 224$\times$224$\times$3 \\
     Low-resolution model & 0.90   &  0.1& 28$\times$28$\times$1\\
     3-nearest neighbor + PCA & 0.80 &  0.05& $224^2 \rightarrow 1000$ \\
     Random forest + PCA & 0.63 & 0.02& $224^2 \rightarrow 1000$ \\
     3-nearest neighbor & 0.75 &  0.4 & $28^2$\\
     Naive Bayes & 0.82 & 0.23& $28^2$\\ \hline
\end{tabular}
 \label{tab:comparison}
 \vspace{-0.1in}
\end{table}
\begin{algorithm}[H]\label{alg:henet}
\caption{HeNet on Intel\textsuperscript{\textregistered} PT}\label{alg:henet}
\begin{algorithmic}[1]
\State \textbf{Goal:} Malware detection.
\State \textbf{Input:} Intel\textsuperscript{\textregistered} PT trace, resizing parameter $m$. 
\State \textbf{Step 1} Convert TNT and TIP packets to pixels of value [$0$, 255]. Denote pixel array by $X$.  
\State \textbf{Step 2} Slice $X$ into $n$ segments, where $n = \frac{L}{m^2}$. $L$ is the length of $X$ and a segment is of length $m^2$. 
\State \textbf{Step 3} Convert each segment to an image of $m \times m$. Denote an image by $I_k$ with $k \in \{1,2,\cdots, n\}$.%, such that $X = (I_1, ..., I_n)$.
\State \textbf{Step 4} Apply low-level deep learning behavior model on $I_k$ and obtain probability of each segment as $p_k$.
\State \textbf{Step 5} Predict the label of $X$ by averaging $(p_1, ...,p_n)$.
\end{algorithmic}
\end{algorithm}

==> intro.tex <==
\section{Motivation}

%malware 
%static, feature engineering, 
%motivates to look into computer vision techniques
%dynamic
%even though effective, black model is not enough. visual explainablity.


Malware is a type of software that possesses malicious characteristics to cause damage to the user, computer or network. Categories of malware include virus, trojan horses, worms, spyware, ransomware and so on. Static and dynamic analyses are two main techniques for malware classification and threat detection. Static analysis is a quick and straightforward way to detect malware without executing the application or monitoring the run time behavior. Signature analysis, the most commonly-used static analysis, extracts code string patterns and matches them with a repository of known malicious patterns. However when the code is obfuscated or morphed, signature matching cannot be applied and becomes less resilient to detect malicious patterns. Moreover the rapid increase of signatures, often in exponential growth, makes the signature matching less efficient and scalable. Dynamic analysis, the other hand, dynamic analysis executes the malware code so that the malicious behaviors can be revealed.  An abnormally behaving process can be flagged from live monitoring. Dynamic analysis observes the ransomware behavior in real time, flags abnormal behaviors, and possesses robustness against obfuscation. However, dynamic analysis can take a longer time than static analysis. Moreover dynamic analysis generates more data which also requires more efforts for feature engineering. 

To enable automated static or dynamic malware classification large scale files, machine learning has been employed and demonstrated strong effectiveness for low-cost detection efficacy. Combined with static analysis, algorithms use the information from the binary file such as function calls or header sections as features and demonstrates to be an effective classifier. ML models to characterize the run time behavior is effective against morphed or obfuscated malware. 


However there are a few drawbacks of the current machine leaning algorithms applied on the malware classification tasks. First of all, manual efforts of feature engineering can be costly and feature extraction may not work on obfuscated malware. Secondly, due to the exponential increase of data as well as unstructured data formats, the scalability and automation of consuming big data in security is desired for the proposed intelligent algorithms. Thirdly, the highly effective deep learning models designed for malware classification can remain black-box with no sensible interpretability, but the capability to explain the prediction done by deep learning algorithm is crucial for security researchers and practitioners before they deploy a model in the wild. Last but not least, the resiliency of the deep learning based algorithms for malware detection is strongly desired, so that these intelligent systems can stand the test of morphed or packed malware or sophisticatedly crafted malware.  

My research explores and addresses the current gaps within security and machine learning domain, particularly extending the recent advances in computer vision to provide different perspectives on security problems and effective solutions for better intelligence-based security. The motivation of using computer vision techniques to solve security problems comes from several directions. First, computer vision provides a visualization on the malware or benignware as a whole, compared with feature extraction techniques only able to extract a certain portion of the information. Deep learning has demonstrated to be superior in large-scale image classification and object detection compared with other approaches. After representing the malware samples as images, transfer learning can be leveraged to accelerate the training without much efforts to find parameters while still inheriting the great classification performance from natural images. Furthermore with visual representation, interpretability models can be applied on the malware images to aid the security practitioners to identify new malware signatures and boost confidence in the deep learning model. With the recent advances in adversarial machine learning in the vision domain, vision-based attack techniques have shown to easily bypass highly effective deep learning models. While such attacks are not explicitly applicable for malware classification, the philosophy of vision-based attacks is transferable to improving the resiliency of deep learning based malware classifier, whose attack surface can be thoroughly studied via computer vision techniques. 

%(add advantages + motivation of my research) divide into four pillars that combines the advances in computer vision to help close the gaps in the research of security and machine learning.
%We discuss the perspectives to formulate malware classification and threat detection as a computer vision problem and juxtapose the resiliency and trustworthiness of computer-vision-based algorithms for security. In malware analysis, static analysis uses malware binary or disassembly code to understand the malicious properties or activities without executing the application. Machine learning combined with static analysis uses the information from the binary file such as function calls or header sections as features and demonstrates to be an effective classifier. However the effort of feature engineering can be costly and feature extraction may not work on obfuscated malware. On the other hand, dynamic analysis executes the malware code so that the malicious behaviors can be revealed. Combined with machine learning, models to characterize the run time behavior is effective against morphed or obfuscated malware. However, dynamic analysis can take a longer time than static analysis. Moreover dynamic analysis generates more data which also requires more efforts for feature engineering. 
% In dynamic analysis, we convert the dynamic behaviors of the malware into time series of images and use a hierarchical ensemble neural network scheme to efficiently and effectively detect run time threats. 
%This tutorial also addresses the security of applying computer vision techniques to malware and threat detection. We evaluate the attack surface of computer-vision-based algorithms for malware detection via investigating the blind spots of the algorithms. We will discuss how to use the generative adversarial networks (GAN) on the run time behaviors converted into images and bypass highly effective malware detectors in a black-box manner. We examine the quality of the GAN-generated malicious samples by comparing the statistical similarity of these samples to real ransomware and benignware. We discuss the potential impact for causative attacks when the training data is poisoned using our proposed method. Understanding the bypass techniques offers very valuable insights to enhance the robustness of malware detectors. 

%Motivation: image representation makes it easy for interpretability and faithful interpretation.
